TwinArch: A Digital Twin Reference Architecture

Background. Digital Twins (DTs) are dynamic virtual representations of physical systems, enabled by seamless, bidirectional communication between the physical and digital realms. Among the challenges impeding the widespread adoption of DTs is the absence of a universally accepted definition and a standardized DT Reference Architecture (RA). Existing state-of-the-art architectures remain largely domain-specific, primarily emphasizing aspects like modeling and simulation. Furthermore, they often combine structural and dynamic elements into unified, all-in-one diagrams, which adds to the ambiguity and confusion surrounding the concept of Digital Twins. Objective. To address these challenges, this work aims to contribute a domain-independent, multi-view Digital Twin Reference Architecture that can help practitioners in architecting and engineering their DTs. Method. We adopted the design science methodology, structured into three cycles: (i) an initial investigation conducting a Systematic Literature Review to identify key architectural elements, (ii) preliminary design refined via feedback from practitioners, and (iii) final artifact development, integrating knowledge from widely adopted DT development platforms and validated through an expert survey of 20 participants. Results. The proposed Digital Twin Reference Architecture is named TwinArch. It is documented using the Views and Beyond methodology by the Software Engineering Institute. TwinArch website and replication package: https://alessandrasomma28.github.io/twinarch/ Conclusion. TwinArch offers practitioners practical artifacts that can be utilized for designing and developing new DT systems across various domains. It enables customization and tailoring to specific use cases while also supporting the documentation of existing DT systems.

==> macros.tex <==
\usepackage{ifthen}
\usepackage{amsthm}
\usepackage{bbm}
\usepackage{xcolor, soul} 
\usepackage[normalem]{ulem}
\usepackage[dvipsnames]{xcolor}
%\usepackage[most]{tcolorbox}
\newcommand{\ra}{$\rightarrow$}

%\newboolean{showcomments}
%\setboolean{showcomments}{false}
%\ifthenelse{\boolean{showcomments}}
%{\newcommand{\nb}[2]{
%      \fcolorbox{black}{yellow}{\bfseries\sffamily\scriptsize#1}
%     {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
%  }
%  \newcommand{\ugh}[1]{\textcolor{red}{\uwave{#1}}} % please rephrase
%   % \newcommand{\ins}[1]{\textcolor{blue}{#1}} % please insert
%   \newcommand{\ins}[1]{\textcolor{blue}{#1}} % please insert
%   \newcommand{\del}[1]{\textcolor{red}{\sout{#1}}} % please delete
%   \newcommand{\chg}[2]{\textcolor{red}{\sout{#1}}{\ra}\textcolor{blue}{\uline{#2}}} % please change
%   %\newcommand{\inspar}[1]{\color{blue}{#1}\color{blue}}
%   \newcommand{\delpar}[1]{\textcolor{red}{#1}}
%   \newcommand{\inspar}[1]{\textcolor{blue}{#1}}
%   \newcommand{\insR}[1]{\textcolor{blue}{#1}} % please insert
%   \newcommand{\delR}[1]{\textcolor{red}{\sout{#1}}} % please delete
%}


\newcommand{\nb}[2]{}
\newcommand{\ugh}[1]{#1}
\newcommand{\ins}[1]{#1}
\newcommand{\del}[1]{}
\newcommand{\chg}[2]{#2}
\newcommand{\delpar}[1]{}
\newcommand{\inspar}[1]{#1}
\newcommand{\insR}[1]{#1}
\newcommand{\delR}[1]{}

\newboolean{showcomments}
\setboolean{showcomments}{true} % change to true/false for review/clean version

\ifthenelse{\boolean{showcomments}}{
  \renewcommand{\nb}[2]{
    \fcolorbox{black}{yellow}{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
  }
  \renewcommand{\ugh}[1]{\textcolor{red}{\uwave{#1}}}
  \renewcommand{\ins}[1]{\textcolor{blue}{#1}}
  \renewcommand{\del}[1]{\textcolor{red}{\sout{#1}}}
  \renewcommand{\chg}[2]{\textcolor{red}{\sout{#1}}{\ra}\textcolor{blue}{\uline{#2}}}
  \renewcommand{\delpar}[1]{\textcolor{red}{#1}}
  \renewcommand{\inspar}[1]{\textcolor{blue}{#1}}
  \renewcommand{\insR}[1]{\textcolor{blue}{#1}}
  \renewcommand{\delR}[1]{\textcolor{red}{\sout{#1}}}
}{}

\newcommand\pat[1]{\nb{Patrizio}{\color{magenta}#1}}
\newcommand\dom[1]{\nb{Domenico}{\color{blue}#1}}



